On the Necessity of World Knowledge for Mitigating Missing Labels in Extreme Classification

Extreme Classification (XC) aims to map a query to the most relevant documents from a very large document set. XC algorithms used in real-world applications learn this mapping from datasets curated from implicit feedback, such as user clicks. However, these datasets inevitably suffer from missing labels. In this work, we observe that systematic missing labels lead to missing knowledge, which is critical for accurately modelling relevance between queries and documents. We formally show that this absence of knowledge cannot be recovered using existing methods such as propensity weighting and data imputation strategies that solely rely on the training dataset. While LLMs provide an attractive solution to augment the missing knowledge, leveraging them in applications with low latency requirements and large document sets is challenging. To incorporate missing knowledge at scale, we propose SKIM (Scalable Knowledge Infusion for Missing Labels), an algorithm that leverages a combination of small LM and abundant unstructured meta-data to effectively mitigate the missing label problem. We show the efficacy of our method on large-scale public datasets through exhaustive unbiased evaluation ranging from human annotations to simulations inspired from industrial settings. SKIM outperforms existing methods on Recall@100 by more than 10 absolute points. Additionally, SKIM scales to proprietary query-ad retrieval datasets containing 10 million documents, outperforming contemporary methods by 12% in offline evaluation and increased ad click-yield by 1.23% in an online A/B test conducted on a popular search engine. We release our code, prompts, trained XC models and finetuned SLMs at: https://github.com/bicycleman15/skim

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}
\usepackage{xspace}
% Mark sections of captions for referring to divisions of figures

% Added by Anirudh
\newcommand{\renee}{Ren\'ee\xspace}
\newcommand{\dexml}{DEXML\xspace}
\newcommand{\alg}{ALG \xspace}
\newcommand{\ani}[1]{{\textcolor{cyan}{#1}}}
\newcommand{\jats}[1]{{\textcolor{brown}{#1}}}

% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}

% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}
\def\rvR{{\mathbf{R}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}
% % vector notation
% \def\vec#1{\mathchoice%
% 	{\mbox{\boldmath $\displaystyle\bf#1$}}
% 	{\mbox{\boldmath $\textstyle\bf#1$}}
% 	{\mbox{\boldmath $\scriptstyle\bf#1$}}
% 	{\mbox{\boldmath $\scriptscriptstyle\bf#1$}}}
% \def\v#1{\protect\vec #1}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sE{{\mathbb{E}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}



% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}
\newcommand{\model}{\textsc{LEVER}\xspace}


\newcommand{\xmark}{\ding{53}}%
% \usepackage{algorithm2e}

% \algnewcommand\algorithmicinput{\textbf{Input:}}
% \algnewcommand\INPUT{\item[\algorithmicinput]}

% \algnewcommand\algorithmicoutput{\textbf{Output:}}
% \algnewcommand\OUTPUT{\item[\algorithmicoutput]}
% Additions by Anirudh Done


\setlength{\tabcolsep}{3pt}

\renewcommand{\L}{\mathcal{L}}
% \newcommand{\E}{\mathcal{E}}
\newcommand{\F}{\mathcal{F}}
% \newcommand{\R}{\mathbb{R}}
\renewcommand{\P}{\mathbb{P}}


\iffalse
% Yash: Including below useful commands in fixed_definitions.tex too. So excluding here to avoid repetition

\newtheorem{assumption}{Assumption}
\newtheorem{theorem}{Theorem}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


\newcommand{\ul}[1]{\underline{#1}}
\fi

==> old_cache.tex <==
% Old dataset descriptions ------------------------------

\textbf{Datasets}: 
We compare our method with existing baselines on 2 publicly available real-world large-scale short-text retrieval datasets described as follows. One is a real clicked dataset and the other one is where we simulate the bias: \\
\begin{enumerate}
    \item \textbf{ORCAS-800K:} This dataset involves retrieving relevant URLs (i.e. the web page corresponding to the URL must be relevant to the search query) for a given short search query. This was curated using clicks from Microsoft's Bing search engine. It contains around 6M short search queries and close to 800K URLs to retrieve from. This dataset exhibits the biases mentioned in earlier sections due to exposure bias and inductive biases of the deployed models. The dataset has a train and test splits, however, both of the splits are biased. To test unbiased performance, we curated a test set using the human labeled test sets available on TREC-19 and TREC-20 DL competitions. More details about the creation of the unbiased test set is in the supplementary.
    \item \textbf{WikiTitlesHierarchy-2M:} The task in this dataset is to map short Wikipedia titles to their respective Wikipedia categories or generalizations of those articles or categories. This dataset was inspired from \cite{buvanesh2024enhancing}, where it is hypothesized that predicting short generic categories is hard for \textit{simple} models like dual encoders. The authors also say that this nature of having a data point relevant to its generic category is reminiscent to that of actual real world short-text retrieval dataset, especially in the domain of ad recommendation. Thus, due to these reasons, it becomes an ideal dataset to test the potential real world applicability of our proposed method. We use a pre-trained BERT dual encoder to simulate the inductive and exposure bias that we observe in real-world clicked datasets. More details about how we simulate the bias and what is the unbiased test set used for evaluation are in the supplementary. This dataset contains 4M titles (data points) and close to 2M categories (labels). This also makes a very good data to do ablations as pointed out in \cite{schultheis2022missing}, since we are controlling the bias.
\end{enumerate}

In addition to above two public datasets, we also evaluate our method on a proprietary dataset, where the task is to map a short search query to its relevant advertiser's short keywords. This dataset was curated using a popular search engine making it an ideal dataset for us, exhibiting severe biases. We call this dataset \textbf{Ads-10M}, having approximately 140M short search queries and around 10M keywords.

Motivation for choice of datasets - (i): short-text, (ii): Availability of an unbiased test set (semi-synthetic). \ani{If you start with the original WikiTitles dataset, you add the subsequent levels to make it clean, and introduce the bias using a pre-trained retriever -- Why didn't you just use the L1 dataset for experiments? That is also an example of a certain kind of bias -- maybe motivate it through real-life bias?}

\textbf{Baselines:} 
We compare our method with different approaches proposed in literature on tackling MNAR bias, LLM based augmentation approaches and recent state-of-the-art XC techniques designed to improve tail label performance. We apply the baselines and our method on top of two recently proposed \textit{base models} for training short-text retrieval models \cite{jain2023renee, gupta2024efficacy}. Below we describe each baseline in more detail and the rationale for choosing each. \\ \\
\textit{Vanilla method:} We train the base model using the biased clicked data only. \\
\textit{Imputation based methods:} These approaches fall into the category of debiasing models using error imputation or error estimations \cite{cite pls}. Recent approaches in short-text retrieval \cite{kharbanda2023gandalf, buvanesh2024enhancing} implicitly use some sort of error imputation or estimation. Gandalf \cite{kharbanda2023gandalf} utilizes random walks ? to impute the training matrix whereas LEVER \cite{buvanesh2024enhancing} imputes using soft scores from a imputation model, similar to classical imputation approaches. \\
\textit{Propensity based methods:} These methods fall into learning unbiased models using propensity scores \cite{saito implicit, tobias2016treatments}. We will use estimation technique discussed in \cite{yash prop paper}. To train base models, we employ the algorithm discussed in \cite{qaraei2021convex}.
We additionally compare these propensity methods where a small quantity of unbiased dataset availability is assumed. \\
\textit{Doubly Robust methods:} Community has proposed doubly robust methods to learn unbiased models \cite{stable DR}, however most of these have been proposed for explicit feedback settings. We cook up a simple doubly robust baseline by combining a imputation and propensity method for our settings. More details about creation of this baseline and how this need not provably be doubly robust \cite{lambda plus 1-lambda propensity paper}is discussed in the supplementary. \\
\textit{LLM/SLM based approaches:} Most LLM based retrieval baselines like \cite{arora2023garmeetsrag} won't be We compare with recently proposed LLM based augmentation approaches \cite{saadfalcon2023udapdr, bonifacio2022inparsdataaugmentationinformation, jeronymo2023inparsv2largelanguagemodels}, however, most of these approaches do not use either meta-data or are not directly optimized for debiasing. More details about the specific implementation we employ can be found in the supplementary. \\

\subsection{Main Results}

Discussion points about results in Table \ref{tab:wikiht-main-table} and \ref{tab:orcas-main-table}
\begin{itemize}
    \item \textbf{Why is it important to look at unbiased results} - Mostly I think there will be cases where the perf. improves in the biased setting but doesn't in unbiased setting, I think this was in Orcas for Gandalf. Imp to call out this. Additionally, looking at biased results might lead to wrongful conclusions about which method performs better. 
    \item \textbf{Why is external knowledge important} - Call out the insufficiency of statistical methods like Gandalf. Imputation models like LEVER learnt on biased data sources are also not fit. We would like UDAPDR to be a bit above LEVER, and make statement like UDAPDR integrated external sources of knowledge, but even the SLM doesn't have that much knowledge which is where our approach comes in - using meta-data to compensate for lack of world knowledge of SLM. 
    \item \textbf{What's wrong with propensity based methods?} Reliable estimation of propensities is challenging as it requires an estimate of the complete ground truth. For ex: JPV used meta data in the form of the category hierarchy. These methods mainly perform inferior due to (i): per label estimates of propensities which is a major assumption and (ii): imprecise estimates of propensities. Nevertheless relying on label frequencies to estimate propensities maybe helpful in certain -- quote some place where Babbar ka method helps. 
    \item \textbf{Combining Imputation and Propensity based - would it work?} We would want this to better than LEVER and Propensity based - to make a statement like it helps, but still we're xx\% better.
    

    
\end{itemize}




% ------ Old related work ------------------------

\textcolor{red}{Extreme classification (XC):}
\begin{itemize}
    \item \textbf{Dual Encoder-based Methods} \citep{gupta2024efficacy, dahiya2023ngame, xiong2021approximate, dahiya2021siamesexml,karpukhin2020dense}, RAMEN (if published)
    \item \textbf{Classifier-based methods} \citep{gupta2022elias, kharbanda2022cascadexml, jain2023renee}
    \item \textbf{Combining both Encoder and Classifier-based methods} (\citep{dahiya2023deep}, UniDec (if preprint is there?)
    \item All of these methods rely on only ground truth to train models, and since the ground truth is biased the quality of trained models is compromised. 
\end{itemize}


\textcolor{red}{Missing labels:}
\begin{itemize}
    \item Creating unbiased loss function in the presence of missing labels. Started with works by \cite{jain2016extreme} (\textcolor{red}{need to fill out some details}). 
    \item  Subsequent works identifying flaws of \cite{jain2016extreme} (i) proposing better propensity models  \citep{schultheis2022missing}, (ii) calling out the separation between the tail and missing labels \citep{qaraei2021convex}
    \item MNAR, MAR, MCAR separation not been made. We are the first ones to call out this separation and utilize LLMs to solve the issue of systematic missing labels in XC.
    
\end{itemize}

\textcolor{red}{Missing not at random (MNAR):}
\begin{itemize}
    \item Position of where items are displayed 
    \item MNAR in XC is not new, has been discussed in the retrieval literature: \citep{benjamin2009collaborativemnar}, This is best paper \citep{joachims2017unbiasedltr}. Something around evaluation in Recommender sys in biased settings: \citep{myttenaere2014ReducingOE, longqi2018unbiasedmnar}. \\
    ----
    \item Initial works on collaborative filtering + MNAR-- \citep{lobatob14mnar}
    \item  \textcolor{red}{VERY RAW - just added papers that maybe relevant}. \citep{hu2022on, ma2021identifiablemnar, chen2023deepgen, hwang2022collaborative, duan2023sslnmar, diego2020debiased}
\end{itemize}

\textcolor{red}{Augmentation based methods in XC:} 
\begin{itemize}
    \item Modeling label correlations-- \citep{buvanesh2024enhancing, kharbanda2023gandalf}
    \item Feature level augmentation (generating new data points by randomly cropping substrings of original data) -- \citep{wei2021towards}
    \item None of these discuss in the context of MNAR, \textcolor{red}{We show the insufficiency of relying on ground truth}
\end{itemize}


\textcolor{red}{Retrieval (knowledge) augmented works:} 
\begin{itemize}
    \item OAK like works

    \item \textcolor{red}{Need to check if these are worth mentioning (just writing from the top my head)} - REALM, Atlas, Retro

    \item QUILL, Knowledge-intensive QA type works: \cite{srinivasan2022quill}, \cite{kang2024knowledge} (uses external knowledge, distillation to SLM, but uses it for question answering generation), \cite{cho-etal-2022-query}: uses external knowledge to do augmentation using LLM -- should also come under Data Augmentation section.
\end{itemize}

\textcolor{red}{LLMs for retrieval works:}
\begin{itemize}
    \item \textbf{Query rewriting:} more works in Table 2 of survey: \cite{wang2023query2doc}, \cite{jagerman2023query}.
    
    \cite{ma2023query} (Uses RL to optimize query rewriting to be beneficial for the final retriever, still uses SLM during test time).
    
    \cite{arora2023garmeetsrag} (Uses LLMs) -- All these methods are expensive during test time retrieval

    \item \textbf{Data augmentation:} \cite{saadfalcon2023udapdr}, \cite{sachan2023questions} -- uses LLMs for data augmentation, however, this won't scale for XC datasets.
    
    \cite{peng2024soft} -- Use SLMs that could work for XC scale, however, we know SLMs lack parametric world knowledge

    RAMEN type works in XC -- does not use LLM but is related to data augmentation.

    \textcolor{red}{All of these works distill generated pairs to an encoder that lacks parameters to absorb diverse knowledge}
\end{itemize}

\textcolor{red}{Knowledge transfer works:} \cite{zhong2023seeking} -- transfers task-specific parameters to a SLM.

% Expensive Oracle - How to match oracle efficiently?
%  ---
% For systematic missing labels
% Definition, Metrics, Datasets
% D1: Lexical similarity / Semantic sim. -
% Solving the missing labels is not possible with current GT. (difference in true and observed distribution)
% Oracle generated test set -- unbiased test sets.

% ----
% Definition of systematic missing labels. 
% Qualitative examples showing BERT based example will not work. -- Examples like Shoes and NIke will not work.
% How do we solve it?
% One of the datasets can be a simulated dataset.
% Other datasets Orcas, EPM -- what's the evaluation metric?
%   a. Propensity thing?
%   b. Oracle thing? (do first)
% 


%  ----
% My questions
% Why is GPT-4 a reliable evaluation?

%%% --------------------------------------------


% Method section Jats Draft


We propose a simple pipeline to de-bias large scale biased datasets. This includes the steps outlined in the following subsections in order.

On a high-level, this first includes aligning a SLM for the task of diverse label generation using the input data point and the loosely associated noisy `world knowledge with it. Note that for different retrieval tasks, label generation might change and hence we need to align the SLM towards the task we are interested in. This is followed by synthetic label generation at scale using noisy world knowledge for every data point in the train set, and finally, training an efficient retriever on this generated data.

\subsection{Creation of silver triplets}
To generate diverse labels using the SLM, one could potentially directly prompt it, however, it has been shown that SLMs lack in following complicated prompt instructions \cite{cite}. Therefore, we align (finetune) our SLM for the task of generating diverse labels given a data point and noisy world knowledge. This also reduces the context length significantly and helps in faster generation since we no longer need to add instructions in the prompt, we only need to provide data point and its world knowledge to the SLM. The task would get baked into the parameters of the SLM. 

However, to align the SLM, we need alignment data. One potential way to do this is to ask a human to annotate (data point, world knowledge, synthetic label) triplets. But this won't scale and is cumbersome. Instead, we could use a powerful LLM like GPT4 to generate these (data point, world knowledge, synthetic label) triplets by prompting accordingly. In this way, we can get enough finetuning data ($\approx 50000$) for aligning the SLM. We include the prompts that we used for this in the supplementary.

\subsection{Finetuning SLM on silver triplets}
Once we collect enough silver triplets, we can begin finetuning the SLM for label generation task. We use the vanilla SFT (Supervised Fine-Tuning) for this, keeping the data point and the world knowledge as the input, and the synhthetic label generated by the LLM as the target response. This is exactly same as the SFT part of RLAIF \cite{cite}. Once we have finetuned the SLM, we can begin to do synthetic label generation at scale. Exact details about training and hardware used is included in the supplementary.

\subsection{Using the SLM for synthetic data generation at scale}
Using the finetuned SLM, we can now generate diverse synthetic labels for every data point in our train set. The SLM can easily scale to millions of data points where a LLM would have taken years for this task. In our experiments, a Llama2-7B was able to scale to datasets having 20M+ data points on a standard GPU server. We provide the time estimates and details about the hardware used in the supplementary.

\subsection{Mapping generated synthetic labels to the actual labels in the dataset}
We could directly use the data point and the generated synthetic label pairs to train the final retriever, however, we perform approximate matching of these generated synthetic label to the actual labels present in the dataset. The reasons to do this are two-fold (1) Using the noisy world knowledge, SLM might generate \textit{out-of-scope} synthetic labels that have no support in the dataset's label distribution. As a result, we might end up training the retriever on unimportant labels (2) This also helps to expand the support of \textit{in-scope} labels by mapping the synthetic label to its minor variants in the label distribution that the SLM might have not generated. For example, a generated synthetic label like ``Populated places in India" could map to labels like ``Villages in India" or ``Towns in India" which would also be relevant to the data point (\textcolor{red}{Think of better example.})

\subsection{Using the synthetic and existing biased data to train task-specific retriever}

Once we have mapped the synthetic labels to the existing labels in the previous step, we combine the synthetic data with the original biased data. Next, we need to distill this combined data to an efficient short-text retriever, e.g. \renee \cite{jain2023renee} or \dexml \cite{gupta2024efficacy}.

\subsection{Training Objective}

\subsection{Inference}


% Method section meta points

Points to emphasize on while writing the method section 
\begin{itemize}

\item GPT-4 Prompt: (a): LLMs like GPT-4 have shown to be useful in retrieval tasks (cite Jimmy Lin papers). Emphasize that they are good for world knowledge. (b): We use LLM to generate a few target examples, where we encode the desirable properties of diversity within our prompt using in-context examples.   Maybe tie this back to Fig. 1, and emphasize that the GPT-4 prompt is built by providing in-context examples from different clusters to ensure diverse generations. 
   
\item Finetuning SLM: GPT-4 cannot scale effectively; hence, we fallback to an SLM. Finetuning is important (cite relevant literature). Additionally, if we have an experiment comparing GPT-4, finetuned SLM, and un-finetuned SLM, we can include a pointer to that as well.
   
\item LLAMA Inference: Task specific meta data is abundant (cite Anshul's papers) and is being leveraged in the forms of Graphs (cite) / training objectives (OAK). SLM does not have as much world knowledge as GPT-4. Conditioning the SLM generation by providing meta-data helps improve performance. For instance, in query to URL mapping task in ORCAS dataset we obtain meta-data in the form of web page text associated with the URL. (The method figure should stick to the same example, and highlight what the meta-data looks like)
   
\item Mapping: An SLM can help access diverse pockets that a retriever might not reach. However, once you reach these diverse points, the mapping can be expanded [lexical variations, minor concept variations], which is where a retriever becomes useful.
\end{itemize}


\textit{Definition of our bias:}

Let $Q$ be a set of semantically similar queries. Assume that $\Bar{Q}$ is a representative query text for the set $Q$.

Let $L_i$ (label cluster) be a set of semantically similar labels. Assume that $\Bar{L_i}$ is a representative label text for the set $L_i$.

Assume that every query in $Q$ is relevant to every label in $L_i$, this also implies that $\Bar{Q}$ is relevant to $\Bar{L_i}$.

We define our bias as:
\begin{itemize}
    \item There is a \textbf{high} probability that queries in $Q$ have a click on labels in $L_i$ if: $\Bar{Q}$ is semantically similar to $\Bar{L_i}$.

    \item There is very \textbf{low} probability that queries in $Q$ have a click on labels in $L_i$ if: $\Bar{Q}$ is semantically dissimilar to $\Bar{L_i}$.
\end{itemize}

Therefore, if any query is semantically dissimilar to any $\Bar{L_i}$, there is a high chance that every label in $L_i$ would be \textit{systematically} missing in the training data i.e. the entire label cluster would be absent.

In our observations, semantically similarity plays a role in the bias due to inductive biases in the deployed models and the exposure biases in the retrieval pipeline employing these models that was used to curate these click logs.


Old into points



Points to cover in intro
\begin{itemize}
    \item \textbf{Scoping the work [Short text retrieval}]: 
    \begin{itemize}
        \item Many recommendation systems involve matching user queries to relevant labels \Jatin{Give an example of user query and label in an application} 
        \item Usually it is accomplished using a retrieval model like dual encoders or recently, extreme classifiers which are trained on large-scale click data curated from search engines
        \item In a lot of applications, user queries are short, and so are the labels, making this matching problem hard due to limited context \Jatin{Give reasons on why should someone work on short-text retrieval}
        \item In this paper, we focus scenario of short-text retrieval due to above reasons \Jatin{This is the problem to work on tbh !!}
    \end{itemize}
    % Large-scale recommendation systems typically consist of two key steps: (i) a retrieval layer that shortlists a set of relevant candidates and (ii) a reranking layer that employs complex architectures to re-rank this shortlist. The retrieval layer is particularly critical because if a relevant item does not appear in the top-K shortlist, it cannot be shown to the user. Our work focuses on improving the retrieval layer. \ani{need a segway into XC}. XC has found applications in numerous real-world scenarios, such as product-to-product recommendation, user query completion, and dynamic search advertising \ani{CITE}. A key challenge in these applications is that user queries are typically short and often require additional contextual knowledge to map them effectively to relevant items. This paper focuses on the retrieval layer, specifically addressing the challenge of handling short text in the context of extreme classification.

    \item What is the problem ? Systematic missing labels, Feedback loops
    \begin{itemize}
        \item However, we observe that training data for retrieval , which is usually curated using large-scale click logs, is heavily biased
        \item That is, certain \textit{groups} of labels (we call it a knowledge concept) are completely missing for a particular search query or in other words, labels are missing not at random for a search query \Jatin{Refine !}
        \item (connect group of labels to a knowledge concept) For example, for search query "exon", labels that cater to the concept of "DNA sequencing" like "label1", "label2", "label3" etc. are all missing, but labels that cater the concept of "definition of exon only" like "wikipedia article of exon", "dicionary definition of exon" is present in the training dataset. (Give one more example of knowledge concept that is missing from the diagram, "knowledge concept3") [all the labels in knowledge cluster are lexically similar !]
        \item simplicity bias, inductive bias of previous deployed model -- bias towards lexically similar knowledge concept with high probability (we observe this is orcas, khud dekhlo agar nhi manna to -- happening feedback loop
        \item we formally characterize this notion of missingness \Jatin{Ask Yash: <some conclusion filler of theory>}
        % \item Thus, certain world knowledge about the search query is always absent \Jatin{tone down a bit !}
        % and consequently, any model trained on these clicked but biased datasets can never predict all the relevant labels, since it would have limited world knowledge \Jatin{Add evidence for this claim - maybe figure 2 ? , also tone this down a bit}
    \end{itemize}

    \item How has the community tackled this problem ? [Missing label literature of MNAR, XC -- propensity solutions -- describe their failure (proof is tables and ablation) -- why can't it solve this problem briefly, Imputation based methods (why can't it solve it briefly), ] [I will talk that these methods do not add world knowledge] \Jatin{emphasize that the goal is to predict all labels fairly, i.e. labels from different knowledge clusters, not be biased towards any single knowledge cluster, and this is where world knowledge is helpful}

    \item LLMs have impressive world knowledge, briefly how people can use it in retrieval (Query2Doc, RRR) (rewrite can tap into new knowledge) can't scale. SLMs directly for rewrite [we want fixed latency]. SLMs for Aug works can scale and provide fixed latency and again could expose to new knowledge (lack parametric knowledge)

    \item Abundant meta-data is available in XC (justify this), however, it is uncurated / unstructured / noisy. [meta-data has knowledge to solve this] Some noisy curated meta-data has been used to solve missing labels \cite{mittal2024graphregularizedencodertraining}. However, such semi-curated types meta-data is either noisy or most of the cases rarely available, as also pointed out in \cite{mittal2024graphregularizedencodertraining}.
    Moreover, if you still use this uncurated meta-data in context, ignoring the latency, RAR works still won;t solve it [mention ablation 2] [even if you relax latency, you still can't solve it using RAR -- increase context length latency for BERT, and not SLM]

    \item In our work we seek to develop a scalable solution to expose relevant labels from different knowledge clusters by making use of an SLM and unstructured meta-data (marking them directly +ve in the ground truth). The meta-data helps compensate for the lack of parametric knowledge. [Emphasizing how different components of the solution are helpful] (i): Scale (SLM Finetuning + final task specific retriever training] (ii): knowledge [counter missing labels my generating relevant labels], [We sort of build a scalable automatic task-specific data curation machine -- it extracts/generates only the relevant knowledge for your task from the meta-data]

    \item{Contibutions}
    \begin{itemize}
        \item Theoretically characterize the notion of missingness that is frequently encountered in XC datasets, and empirically demonstrate the harmful effects of using biased datasets.
        \item Propose a method to effectively leverage the capabilites of LLMs and unstructured data to debias large-scale retrieval datasets. Our experiments demonstrate that leveraging our pipeline to debias datasets results in \ani{xx\%} gains on \textit{unbiased} datasets. \ani{Need to highlight the flexibility of the method - it's algorithm agnostic, just extracts most valuable information from the unstructured data to mitigate the systematic missingness}
        \item Conduct extensive ablations to validate our design choices
        \item Validate the efficacy of our method on a sponsored search application where the task is of matching user queries to advertiser bid keywords. Our experiments demonstrate \ani{yy\%} gains in \ani{XX metrics}.
    \end{itemize}
    
\end{itemize}

% 
% Experimental Results Jatin draft

\textbf{Datasets}: We evaluate our method and the competing baselines on two large-scale short-text datasets, namely LF-Orcas-800K and LF-WikiTitlesHierarchy-2M. The task in LF-Orcas-800K dataset is to predict relevant URLs from a given short search query. This dataset was curated using user-clicks from a popular search engine, and thus exhibiting extreme biases \textcolor{red}{(what biases exactly ?)}, making it an ideal dataset to test performance. Since every URL points to a web page, we employ that web page as our unstructured knowledge source or meta-data \textcolor{red}{(Decide what to call meta-data: unstructured meta-data sounds good to me :p, open for suggestions)}. LF-WikiTitlesHierarchy-2M on the other hand caters to the task of predicting all relevant Wikipedia categories for a given short Wikipedia title, which was created keeping in mind the real-world task of query-to-ad keyword prediction \cite{buvanesh2024enhancing}.
We simulate the systematic missingness bias in this dataset using a pretrained model. 
Every Wikipedia title comes along with the entire article body text about that title, which we use here as our meta-data.
We additionally test our method on real-world proprietary dataset collected from user-clicks using a search engine. The task is short search query-to-ad keyword prediction. This dataset again, due to its nature of curation, exhibits the same extreme biases \textcolor{red}{(what biases exactly ?)} we talked about earlier, making it a perfect dataset to test the real-world applicability of our method on large-scale.  We call this dataset LF-Query2Keyword-10M. Every ad keyword is usually supplied with an ad campaign \textcolor{red}{(describe this ad campaign more)} information, which we employ as our unstructured meta-data for this dataset.
More details about the datasets in general, their curation details, meta-data, statistics and simulation of bias can be found in the appendix. 



    % \item There should be a method that promotes exposure to new knowledge concepts/clusters [this is our main observation to solve the MNAR problem] 

    % \item{\textbf{Motivation for world knowledge}} 
    %     \begin{itemize}
    %         \item \textbf{Defining knowledge clusters} To highlight the challenges posed in the short text retrieval scenario we consider the example of the ORCAS dataset where the task is that of matching user queries to web page URLs. Here consider a query \textit{exon } \ani{INCOMPLETE}
    %         \item \textbf{Highlighting that knowledge clusters systematically go missing} Refer to the figure and show how certain concepts are absent in the data. What is present is rather some kind of \textit{simple} matches - define the term \textit{simplicity bias}. Maybe end with something like, note that this bias arises due to a combination of several underlying biases which have already been discussed in literature (position bias: users tending to click stuff on towards the top + exposure bias: if a relevant item is not exposed no chance of getting click)
    %         \item \textbf{Theory connection}: Briefly state something like - we characterize this notion of missingness concretely (\ani{ASK YASH: ask what can be stated here})
    %         \item \textbf{Implications of training a retriever on such missing data}
    %         \item \textbf{Ineffectiveness of other solutions} Very briefly highlight the limitations of RAG (since world knowledge is being discussed), propensity (since biases are being discussed), and augmentaiton in general.

    %         End with world knowledge is the way to go :P
    %         \ani{Just for people who are against use world knowledge - maybe we can somewhere add that world knowledge in the form of web-scraped data \cite{aggarwal2023semsupxc}, manually curated data \cite{mohan2024oak} is already being leveraged. Make the point about unstructured data in a proper way - Emphasize that unstructured data is plenty and needs to be leveraged}

    %     \end{itemize}


    % \item \textbf{LLMs as a solution to world knowledge + Scaling up} LLMs have shown impressive capabilites in the IR space - specially on re-ranking tasks \ani{CITE jimmy lin papers}. However, their use in large-scale retrieval tasks is still limited \ani{check / cite}. Our goal is to leverage the world knowledge capabilites of LLMs to solve the \textit{simplicity bias} issue. Recipe to scale involves finetuning an SLM on task-specific instructions obtained from an LLM, and then using unstructured meta-data to generate concepts from missing knowledge clusters.


% \textcolor{red}{Why did we need to do something:}
% \begin{itemize}
%     \item Missing labels are abound in real-world large-scale datasets. In tasks such as extreme classification (XC), where the scale of labels in hundreds of million, labels are \textit{systematically} missing i.e. certain \textit{category} of labels for some \textit{category} of data points are completely missing or data points are biased towards certain \textit{category} of labels only. As a result, XC models trained on these biased datasets result in biased predictions, that are unable to predict the missing labels.
%     \item Missing labels is an important and well-studied problem in XC \citep{jain2016extreme, schultheis2022missing}. Labels can go missing in different ways - MNAR, MAR, MCAR. \textcolor{red}{CHECK:} However, XC literature has not made this differentiation between the different forms of missing labels.

%     \item We make the observation (\textcolor{red}{Need to think what is the observation}) that external world knowledge is crucial in solving systematic missing labels problem. Our findings reveal most of the current approaches (that solely rely on ground truth statistics \citep{buvanesh2024enhancing, kharbanda2023gandalf}) are insufficient to tackle the systematic nature of missing labels in XC scenarios.

%     \item To address this world knowledge problem, retrieval augmentation \cite{} can be viable option, however their use involves increasing the inference cost significantly (due to increased context lengths), thereby making its use limited in production scenarios.

%     % \item In this work, we show that for the specific kind of missing labels that occur in XC tasks . We evaluate the effectiveness of existing methods that leverage ground truth to compensate for missing labels, as proposed in prior research \citep{kharbanda2023gandalf, buvanesh2024enhancing}.
    
% \end{itemize}
% % Missing labels is a big problem in extreme classification (XC) tasks.

% \textcolor{red}{How did we address the challenges:} Since world knowledge is important to MNAR problem, a natural solution could be LLMs (cite some LLMs are knowledge bases work). 
% \begin{itemize}
%     \item Using LLMs for world knowledge during test time -- past works have used LLMs, but their inference cost is high (citing rewrite works)
%     \item Using LLMs to expose retrieval to world knowledge (during training) -- past works have explored data augmentation as a way to render world knowledge to efficient retrievers, but, they have not been explored in MNAR scenarios. More importantly, these methods cannot scale to XC datasets. 
%     \item Using SLMs to expose retrieval to world knowledge (during training) -- there are works that do this, but, we know SLMs lack parametric world knowledge
%     \item Using SLMs + meta information -- there is a work that does this, however, does this for answer generation and uses SLM at test time, no MNAR thingy there (SLM is still costly for low latency requirements like search and recommendation)
%     \item In XC, datasets usually have abundant meta-information that can be used to solve world knowledge problem and consequently solve MNAR, however, due to their unstructured format, they cannot be readily in existing XC learning algorithms. One way is to use the meta-information during test time by appending it to the context, however, this increases the latency. OAK and RAMEN do use noisy form of consumable external meta-information, however, (a) they do not directly solve MNAR (b) there linkages can be noisy (c) these \textit{meta-information linkages} need not be present in all scenarios.
%     % \item Some recent works have explored LLMs/SLMs for improving retrieval, specifically for query rewriting (cite), however, they do not address this MNAR problem. Additionally, there is a high cost involved in inferencing LLMs during test time, leaving these approaches useless in low latency production scenarios.  
    
% \end{itemize}

% \textcolor{red}{What are the contributions:}
% \begin{itemize}
%     % \item Propose a way to quantify the extent to which the problem of systematic missing labels is solved, using which we show the effectiveness of incorporating world-knowledge using LLMs.
%     \item Propose a method (using data augmentation) to effectively distil external world knowledge from SLM + \textit{unstructured/uncurated} meta-information into an XC layer that has high capacity, and low inference costs which is critical in real-world application scenarios.
%     \item We make the observation, that external world knowledge is imperative to solve MNAR, we prove this using Amit's idea (there are empty pockets when there are tail data points and tail labels, rich getting richer)
    
% \end{itemize}


\begin{table}[h!]
\caption{\ani{Refactor: \dexml and \renee Results for \orcas}}
\centering
\begin{tabular}{clGGcc}
\toprule
& & \multicolumn{4}{c}{\orcas} \\
\cmidrule(r){3-6} 
& &  \multicolumn{2}{G}{Biased} & \multicolumn{2}{c}{Unbiased} \\
& & R@25 & R@100 & R@25 & R@100 \\
\midrule
& \dexml & & & &  \\
\midrule
\multirow{2}{*}{\textcircled{1}} &+ Gandalf & & & &  \\
&+ LEVER & & & &  \\
\midrule
\multirow{2}{*}{\textcircled{2}}&+ IPS & & & &  \\
&+ LEVER + IPS & & & &  \\
\midrule
\multirow{1}{*}{\textcircled{3}}&+ \slmaug & & & &  \\
\midrule
&+ \alg (Ours) & & & &  \\
\midrule
\midrule
&\renee & & & &  \\
\midrule
\multirow{2}{*}{\textcircled{1}} &+ Gandalf & & & &  \\
&+ LEVER & & & &  \\
\midrule
\multirow{2}{*}{\textcircled{2}}&+ IPS & & & &  \\
&+ LEVER + IPS & & & &  \\
\midrule
\multirow{1}{*}{\textcircled{3}}&+ \slmaug & & & &  \\
\midrule
& + \alg (Ours) & & & &  \\

\bottomrule
\end{tabular}
\label{tab:orcas-main-table}
\end{table}



\begin{table}[h!]
\caption{\ani{Refactor: \dexml and \renee Results for \wiki. }}
\centering
\begin{tabular}{clGGcc}
\toprule
& & \multicolumn{4}{c}{\wiki} \\
\cmidrule(r){3-6} 
& &  \multicolumn{2}{G}{Biased} & \multicolumn{2}{c}{Unbiased} \\
& & R@25 & R@100 & R@25 & R@100 \\
\midrule
& \dexml & & & &  \\
\midrule
\multirow{2}{*}{\textcircled{1}} &+ Gandalf & & & &  \\
&+ LEVER & & & &  \\
\midrule
\multirow{2}{*}{\textcircled{2}}&+ IPS & & & &  \\
&+ LEVER + IPS & & & &  \\
\midrule
\multirow{1}{*}{\textcircled{3}}&+ \slmaug & & & &  \\
\midrule
&+ \alg (Ours) & & & &  \\
\midrule
\midrule
&\renee & & & &  \\
\midrule
\multirow{2}{*}{\textcircled{1}} &+ Gandalf & & & &  \\
&+ LEVER & & & &  \\
\midrule
\multirow{2}{*}{\textcircled{2}}&+ IPS & & & &  \\
&+ LEVER + IPS & & & &  \\
\midrule
\multirow{1}{*}{\textcircled{3}}&+ \slmaug & & & &  \\
\midrule
& + \alg (Ours) & & & &  \\

\bottomrule
\end{tabular}
\label{tab:main-table}
\end{table}


% Jatin's Baseline section




We applied our generally applicable method on top of two strong and diverse \textit{base} XC models, specifically a state-of-the-art extreme classifier \renee \cite{jain2023renee} and a recently proposed strong dual-encoder \dexml \cite{gupta2024efficacy}.
We then compare our method with several error imputation \cite{steck2013evaluation} based approaches proposed in XC literature, namely LEVER \cite{buvanesh2024enhancing} and Gandalf \cite{kharbanda2023gandalf}. We also compare with inverse propensity re-weighting/scoring (IPS) \cite{tobias2016treatments, saito2020unbiased} approaches in XC \cite{schultheis2022missing, jain2016extreme}, and a heuristic doubly robust \cite{li2023stabledr} estimation baseline, constructed from \cite{buvanesh2024enhancing, jain2016extreme}. Finally, we compare our approach with a slightly modified version of SLM-based augmentation methods \cite{saadfalcon2023udapdr, jeronymo2023inparsv2largelanguagemodels, bonifacio2022inparsdataaugmentationinformation} for our use-case. 
We apply each of the competing baseline on top of the two \textit{base} XC models, namely \renee and \dexml. \textcolor{red}{(Emphasize more why these baselines are strong!! maybe we do that in intro or related work ? its not coming out clearly what we are doing is amazing :p !)} Exact details about the implementation of each of these baselines can be found in the appendix.

% To assess unbiased retrieval performance, one requires access to an unbiased test dataset. In case of LF-Orcas-800K, we could curate a small unbiased test dataset using the human labeled test sets available on TREC-19 and TREC-20 Deep Learning competitions \cite{craswell2020overview}. For LF-WikiTitlesHierarchy-2M, since we simulate the bias, we already have access to the complete unbiased test set. Finally, for LF-Query2Keyword-10M, we employ a proprietary filter model which measures a relevance of a predicted (query, keyword) pair. More details about the creation of the unbiased test set for LF-Orcas-800K and the proprietary filter model is in the appendix. \\
% For experiments with LF-Orcas-800K and LF-WikiTitlesHierarchy-2M, we measure $Recall@K$ with $K=25$ and $K=100$ against the unbiased test set. We use higher values of $K$ (as opposed to $K=5,10$) since we want to measure the retrieval performance and not re-ranking (that focuses on measuring $Precision@K$ or $Recall@K$ for lower values of $K$). \textcolor{red}{(Motivate somewhere in the beginning that if retrieval is broken, re-ranking can't do anything: Our approach is orthogonal to re-ranking, you can always apply re-ranking on top of our trained retrievers to get better precision -- Also say in the beginning that people have not focused on solving retrieval pipeline, they only focus on fixing precision)} Additionally in table \ref{}, we measure biased test performance for our method and baselines, showcasing the cautionary tale if we rely on biased test performance to decide to deploy models in production.
% For experiments with LF-QueryToKeyword-10M, we measure $Hits@100$ i.e. the pairs marked relevant by the proprietary filter model in top-100 predictions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Here we discuss some interesting observations in our main results i.e. in Table \ref{tab:main-table}. \Jatin{make the point of large scale evaluation more prominent i.e. we don't use any academic XC datasets, we use large-scale ones to show the effectiveness of our method on large-scale}
% 
% \textbf{\alg outperforms all baselines.} On both the public short-text retrieval datasets, \alg, when used with any XC model \Jatin{this makes \alg generally applicable}, outperforms all the baselines when measured on unbiased test sets. In \orcas, where the clicks exhitibt the real-world large-scale systematic missingness bias we aim to address, \alg significantly outperforms the closest baseline XYZ by more than \textbf{X} absolute points in terms of $Recall@100$ (and \textbf{Y} absolute points in $R@25$). On a similar note in \wiki, \alg outperforms the closest competitor by more than X absolute points in terms of $Recall@100$. \Jatin{update this !}


==> tables/old_tables.tex <==
\begin{table}[htbp]
    \centering
    \caption{Unbiased performance of different methods against the simulated bias on LF-WikiTitlesHierarchy-2M}
    \begin{tabular}{llcccc}
        \toprule
        \multirow{2}{*}{} & \multirow{2}{*}{} & \multicolumn{4}{c}{Unbiased} \\
        \cmidrule(lr){3-6} 
         &  &  R@5 & R@10 & R@25 & R@100 \\
        \midrule
        \multirow{2}{*}{Base Retrievers} & \renee & 5.90 &  7.83 & 9.84 & 12.79 \\
         & \dexml & 6.16 & 8.27 & 10.87 & 15.02 \\
        \midrule
        \multirow{4}{*}{Imputation} & \renee + Gandalf & 6.28 & 8.46 & 11.10 & 15.30 \\
         & \renee + LEVER & 6.47 &  8.59 & 11.15 & 15.98 \\
          & \dexml + Gandalf & 6.14 & 8.23 & 10.73 & 15.01 \\
         & \dexml + LEVER  &  Running & - & - \\
        \midrule
        \multirow{2}{*}{Propensity Wt.} & \renee + IPS & 6.77 &  9.11 & 11.98 & 16.64 \\

        & \dexml + IPS & 5.97 &  8.10 & 10.92 & 15.92 \\
        \midrule
        \multirow{2}{*}{DR*} & \renee + LEVER + IPS & 6.78 &  9.22 & 12.61 & 19.19 \\
        & \dexml + LEVER + IPS & TODO &  - & - & - \\
        \midrule
        \multirow{1}{*}{LLM based methods} 
        & UDAPDR & \dexml:Running & - & - & - \\
        \midrule
        \multirow{2}{*}{Ours}  & \renee + Ours & 7.10 & 11.00 & 17.30 & 28.10 \\
        & \dexml + Ours & 7.56 & 11.13 & 16.59 & 25.42 \\
        \bottomrule
    \label{tab:wikiht-main-table}
    \end{tabular}
    
\end{table}


% 30.24	36.01	42.91	48.51	52.11


\begin{table}[htbp]
    \centering
    \caption{Unbiased performance of different methods against the real-world bias (due to exposure/inductive bias) of LF-Orcas-800K dataset}
    \begin{tabular}{llcccc}
        \toprule
        \multirow{2}{*}{} & \multirow{2}{*}{} & \multicolumn{4}{c}{Unbiased} \\
        \cmidrule(lr){3-6} 
         &  &  R@5 & R@10 & R@25 & R@100 \\
        \midrule
        \multirow{2}{*}{Base Retrievers} & \renee & 34.23 &  40.25 & 47.61 & 59.82 \\
         & \dexml & 26.80 & 34.39 & 41.45 & 51.31 \\
        \midrule
        \multirow{4}{*}{Imputation} & \renee + Gandalf & 28.38 & 33.00 & 37.60 & 45.11 \\
         & \renee + LEVER & 32.33 &  41.82 & 49.47 & 59.95 \\
          & \dexml + Gandalf & 30.24 & 36.01 & 42.91 & 52.11 \\
         & \dexml + LEVER  &  28.60 & 34.92 & 41.64 & 52.76 \\
        \midrule
        \multirow{2}{*}{Propensity Wt.} & \renee + IPS & 24.02 &  28.50 & 31.58 & 40.21 \\
        & \dexml + IPS & Running &  - & - & - \\
        \midrule
        \multirow{2}{*}{DR*} & \renee + LEVER + IPS & 27.48 &  33.21 & 39.92 & 46.81 \\
        & \dexml + LEVER + IPS & TODO:A &  - & - & - \\
        \midrule
        \multirow{1}{*}{LLM based methods} & UDAPDR & 29.49 & 38.66 & 45.39 & 57.57 \\
        \midrule
        \multirow{2}{*}{Ours}  & \renee + Ours & 31.50  & 42.18 & 57.25 & 70.92 \\
        & \dexml + Ours & 31.82 & 42.53 & 54.58 & 68.95 \\
        \bottomrule
    \label{tab:orcas-main-table}
    \end{tabular}
    
\end{table}


% GAR Meets Rag on Orcas

% WikiHierarchy
% \dexml + 
% LEVER
% GAndalf
% Propensity -- Read Amit's paper, think how to intregate
% DR

% Orcas
% \dexml + 
% LEVER
% GAndalf
% Propensity -- Read Amit's paper, think how to intregate
% DR




\subsection{Ablations}

\textbf{Effect of size of SLM on final retrieval performance}. Table \ref{tab:slm-size-ablation} Experiment with some (\textcolor{red}{sizes TBD}) 500M, 1B, 7B models. == msmarco (1B, 7b)

\begin{table}[htbp]
    \centering
    \caption{Effect of size of SLM on final retrieval performance. Evaluations were done on an unbiased test set}
    \begin{tabular}{lcc}
        \toprule
        \multirow{2}{*}{}  & \multicolumn{2}{c}{Orcas} \\
        \cmidrule(lr){2-3} 
         &  R@25 & R@100 \\
        \midrule

        \renee + Phi-2B   & DONE: J & -  \\
        \renee + LLAMA-7B   & 54.58 & 68.95 \\
        \bottomrule
        \label{tab:slm-size-ablation}
    \end{tabular}
\end{table}

\textbf{Effect of  meta-data (M)}: Table \ref{tab:metadata-effect-ablation} shows the effect of using meta-data \textcolor{red}{TODO describe trends}. Have on both datasets
\begin{table}[h!]
    \centering
    \caption{Effect of meta-data on the performance of the retriever}
    \begin{tabular}{lccccc}
        \toprule
         Retriever & Meta-data & \multicolumn{2}{c}{LF-WikiTitle-Hierarchy} & \multicolumn{2}{c}{Orcas} \\
        \cmidrule(lr){3-4} \cmidrule(lr){5-6}
         &  & R@25 & R@100 & R@25 & R@100 \\
        \midrule
        \dexml & \xmark & TODO:A & - & - & -\\
        \renee & \xmark & DONE:J & - & - & -\\
        \dexml & \cmark & TODO:A & - & - & -\\
        \renee & \cmark & DONE:J & - & - & -\\
        \bottomrule
        \label{tab:metadata-effect-ablation}
    \end{tabular}
\end{table}

\textbf{Effect of  meta-data}:

\textbf{RAG doesn't work directly (M) : Concatenating the meta-data instead of using it to debias}:  Table \ref{tab:in-context-vs-debiased-ablation} shows trends. Two points to highlight: (i): the inference time blow up, and (ii): the performance is still inferior - debiasing is important, just passing stuff in-context won't work out. 
\begin{table}[h!]
    \centering
    \caption{Performance and Inference Time Comparison}
    \begin{tabular}{llcccccc}
        \toprule
        & & \multicolumn{3}{c}{LF-WikiHierarchy-Title} & \multicolumn{3}{c}{-} \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-8}
        & & R@25 & R@100 & Inf. Time & R@25 & R@100 & Inf. Time \\
        \midrule
        % \multirow{2}{*}{\dexml} & In Context & todo:a & - & - & - & - & - \\
        %                        & ours   & DONE:A & - & - & - & - & - \\
        %                        % & ours + In context & TODO: LOW PRI: J  & - & - & - & - & - \\
        % \midrule
        \multirow{2}{*}{\renee} & Biased + In Context & DONE:A & - & - & - & - & - \\
                               & Debiased (nothing in context)  & DONE:A & - & - & - & - & - \\
                               & Debiased + In context & TODO: J  & - & - & - & - & - \\
        \bottomrule
    \label{tab:in-context-vs-debiased-ablation}
    \end{tabular}
\end{table}


\textbf{Effect of amount of synthetic data}; This needs some thought; it's probably not so nice to show a flat line - exact details need to be formalized - Jatin had some preliminary thoughts - 10, 40, 80, 100 -- Start w/ 10 -- Sachin -- Orcas - \renee - To create datasets + Do runs, Which metrics to show in retrieval -- Coverage / MRR / Hits? \textbf{DONE}

\textbf{Other benefits of the data we provide}: \textcolor{red}{How important? - describe preliminary experiments - deriving propensities from original unbiased data  in WikiHierarchy} Deriving propensities using this data and then training models - need to think what to compare against: TODO: A

\textbf{Effect of filter}:  LLAMA Filter w/ and w/o

% \textbf{Effect of retriever used to map on to the original label space}: Low priority - maybe with NGAME and \dexml?
